Type-Safe Feature-Oriented Product Lines

A feature-oriented product line is a family of programs that share a common set of features. A feature implements a stakeholder's requirement, represents a design decision and configuration option and, when added to a program, involves the introduction of new structures, such as classes and methods, and the refinement of existing ones, such as extending methods. With feature-oriented decomposition, programs can be generated, solely on the basis of a user's selection of features, by the composition of the corresponding feature code. A key challenge of feature-oriented product line engineering is how to guarantee the correctness of an entire feature-oriented product line, i.e., of all of the member programs generated from different combinations of features. As the number of valid feature combinations grows progressively with the number of features, it is not feasible to check all individual programs. The only feasible approach is to have a type system check the entire code base of the feature-oriented product line. We have developed such a type system on the basis of a formal model of a feature-oriented Java-like language. We demonstrate that the type system ensures that every valid program of a feature-oriented product line is well-typed and that the type system is complete.

==> sec/AuxDefPL.tex <==
\begin{figure*}
\begin{center}
\begin{tabular}{l l}
\textit{Field lookup} & \hfill \fbox{$\mathit{fields}(\overline{\qtm{\Phi}{C}}, \qtm{\Phi}{C}) = \overline{\mol{C~f}\fieldsep}$} \\[2ex]
\multicolumn{2}{c}{
$\mathit{fields}(\overline{\qtm{\Phi}{C}}, \qtm{\Phi}{Object}) = \bullet\fieldsep$
}\\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{class C extends D \{\ } \mol{C~f;}\ \mol{M}\ \masf{\}} \qquad \mathit{fields}(\mathit{last}(\masf{D},\man{\Psi}),\man{\Psi}) = \overline{\f\fieldsep}
}
{
\mathit{fields}(\qtm{\Phi}{C},\man{\Psi}) = \f_{1},\mol{C~f}\fieldsep \ldots\fieldsep \f_{n},\mol{C~f}\fieldsep
}$
}\\[4ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{refines class C \{\ } \mol{C~f;}\ \mol{M}\ \masf{\}} \qquad \mathit{fields}(\mathit{pred}(\qtm{\Phi}{C},\man{\Psi}),\man{\Psi}) = \overline{\f\fieldsep}
}
{
\mathit{fields}(\qtm{\Phi}{C},\man{\Psi}) = \f_{1},\mol{C~f}\fieldsep \ldots\fieldsep \f_{n},\mol{C~f}\fieldsep
}$
}\\[4ex]
\multicolumn{2}{c}{
$
\mathit{fields}(\overline{\qtm{\Phi}{C}},\man{\Psi}) = \mathit{fields}(\man{\Phi}_1.\masf{C}_1,\man{\Psi})\fieldsep \ldots\fieldsep \mathit{fields}(\man{\Phi}_n.\masf{C}_n,\man{\Psi})\fieldsep
$
}\\[4ex]
\textit{Method type lookup} & \hfill \fbox{$\mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \overline{\overline{\masf{B}} \fct \masf{B$_0$}}$} \\[2ex]
\multicolumn{2}{c}{
$\mathit{mtype}(\masf{m},\qtm{\Phi}{Object},\man{\Psi}) = \bullet$
}\\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{class C extends D \{\ } \mol{C~f};\ \mol{M}\ \masf{\}} \qquad \masf{B$_0$ m(\ol{B~x}) \{ return t; \}} \in \mol{M}
}
{\mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \mathit{mtype}(\masf{m},\mathit{last}(\masf{D},\man{\Psi}), \man{\Psi}), \mol{B} \fct \masf{B$_0$}}$
}\\[4ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{class C extends D \{\ } \mol{C~f};\ \mol{M}\ \masf{\}} \qquad \masf{m} \mbox{ is not defined in } \mol{M}
}
{\mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \mathit{mtype}(\masf{m},\mathit{last}(\masf{D},\man{\Psi}), \man{\Psi})} $
}\\[4ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{refines class C \{\ } \mol{C~f};\ \mol{M}\ \masf{\}} \qquad \masf{B$_0$ m(\ol{B~x}) \{ return t; \}} \in \mol{M}
}
{\mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \mathit{mtype}(\masf{m},\mathit{pred}(\qtm{\Phi}{C},\man{\Psi}), \man{\Psi}), \mol{B} \fct \masf{B$_0$}} $
}\\[4ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{CT}(\qtm{\Phi}{C}) = \masf{refines class C \{\ } \mol{C}\ \mol{f};\ \mol{M}\ \masf{\}} \qquad \masf{m} \mbox{ is not defined in } \mol{M}
}
{\mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \mathit{mtype}(\masf{m},\mathit{pred}(\qtm{\Phi}{C},\man{\Psi}), \man{\Psi})} $
}\\[4ex]
\multicolumn{2}{c}{
$\mathit{mtype}(\masf{m},\overline{\qtm{\Phi}{C}}, \man{\Psi}) = \mathit{mtype}(\masf{m},\man{\Phi}_1.\masf{C}_1, \man{\Psi}), \ldots, \mathit{mtype}(\masf{m},\man{\Phi}_n.\masf{C}_n, \man{\Psi})$
}\\[4ex]
\multicolumn{1}{l}{\textit{Valid class introduction}} \hfill & \hfill \fbox{$\mathit{introduce}(\qtm{\Phi}{C})$} \\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\nexists\, \man{\Psi}\, :\, (\mathit{CT}(\qtm{\Psi}{C}) = \masf{class C}\ldots\ \wedge\ \man{\Phi} \ne \man{\Psi}\ \wedge\ \neg\mathit{exclusive}(\man{\Phi},\man{\Psi}))
}
{\mathit{introduce}(\qtm{\Phi}{C})}$
}\\[4ex]
\textit{Valid field introduction} & \hfill \fbox{$\introduceF{f}{C}{\Phi}{\Psi}$} \\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\forall\, \qtm{\Phi}{C} \in \overline{\qtm{\Phi}{C}}\, :\, ( \forall\, \mol{E~h} \in \mathit{fields}(\qtm{\Phi}{C}, \man{\Psi})\, :\, \masf{f} \notin \mol{h})
}
{\introduceF{f}{C}{\Phi}{\Psi}}$
}\\[4ex]
\textit{Valid method introduction} & \hfill \fbox{$\introduceF{m}{C}{\Phi}{\Psi}$} \\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\forall\, \qtm{\Phi}{C} \in \overline{\qtm{\Phi}{C}}\, :\, \mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) = \bullet
}
{\introduceF{m}{C}{\Phi}{\Psi}}$}\\[4ex]
\multicolumn{1}{l}{\textit{Valid class refinement}} \hfill & \hfill \fbox{$\mathit{refine}(\qtm{\Phi}{C})$} \\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\mathit{RT}(\masf{C},\man{\Phi}) = \overline{\man{\Psi}}, \man{\Phi}, \overline{\man{\Omega}} \qquad \mathit{always}(\man{\Phi},\masf{C}) \mbox{ in } \overline{\man{\Psi}}
}
{\mathit{refine}(\qtm{\Phi}{C})}$
}\\[4ex]
\textit{Valid method overriding} & \hfill \fbox{$\overrideF{m}{C}{\Phi}{\mol{C} \fct \masf{C$_0$}}{\Psi}$} \\[2ex]
\multicolumn{2}{c}{
$\dfrac{
\begin{array}{c}
\mathit{always}(\man{\Psi},\masf{C.m}) \\
\forall\, \qtm{\Phi}{C} \in \overline{\qtm{\Phi}{C}}\, :\, (\forall\, \mol{B} \fct \masf{B$_0$} \in \mathit{mtype}(\masf{m},\qtm{\Phi}{C}, \man{\Psi}) \, : \, \mol{C} = \mol{B} \ \wedge \ \masf{C$_0$} = \masf{B$_0$})
\end{array}
}
{\overrideF{m}{C}{\Phi}{\mol{C} \fct \masf{C$_0$}}{\Psi}}$
}\end{tabular}
\end{center}
\caption{Auxiliary definitions of \ffjpl.}
\label{fig:auxpl}
\end{figure*}

==> sec/altpred.tex <==
Function $\mathit{mspec}$ receives a list of features that introduce or refine a certain class and determines the features that apply the most specific, alternative refinements (or introductions, in the case there are no refinements). That is, each feature in the result list excludes every other feature in the list. The first rule is just a ``wrapper'' that invokes the actual function with the input list and an empty list that is used to store the alternative features in each step. The next two rules traverse the input list, and the first of the two stores the features that are alternative (using $\mathit{exclusive}$). The fourth rule terminates the recursion and returns the stored features.

\begin{center}
\begin{tabular}{l l}
\multicolumn{2}{c}{
$\mathit{mspec}(\overline{\man{\Phi}}) = \mathit{mspec}(\overline{\man{\Phi}},\bullet)
$
}\\[4ex]
$\dfrac{
\mathit{exclusive}(\man{\Phi}_n,\overline{\man{\Psi}}) \qquad \overline{\man{\Omega}} = \man{\Phi}_1, \ldots, \man{\Phi}_{n-1} \qquad \overline{\man{\Pi}} = \man{\Phi}_n,\overline{\man{\Psi}}
}
{
\mathit{mspec}(\overline{\man{\Phi}},\overline{\man{\Psi}}) = \mathit{mspec}(\overline{\man{\Omega}},\overline{\man{\Pi}})
}$
}\\[4ex]
\multicolumn{2}{c}{
$\dfrac{
(\man{\Phi}_n,\overline{\man{\Psi}}) \notin \mathit{dom}(\mathit{exclusive}) \qquad \overline{\man{\Omega}} = \man{\Phi}_1, \ldots, \man{\Phi}_{n-1}
}
{
\mathit{mspec}(\overline{\man{\Phi}},\overline{\man{\Psi}}) = \mathit{mspec}(\overline{\man{\Omega}},\overline{\man{\Psi}})
}$
}\\[4ex]
\multicolumn{2}{c}{
$\mathit{mspec}(\bullet,\overline{\man{\Psi}}) = \overline{\man{\Psi}}
$
}
\end{tabular}
\end{center}


